Extending Pathwise Gradients to Discrete Random Variables via Finite-Order Relaxation

Pathwise gradients are preferred for continuous random variables because they are unbiased, low variance, and work with a single sample. For discrete variables, however, the pathwise identity cannot generally be exact for every differentiable function. We propose a general framework to construct finite-order exact pathwise gradient estimators for a range of common discrete variables such as Poisson. The estimator is the least-norm solution among all solutions that are unbiased for polynomials of degree at most. The resulting estimators preserve the hard forward sample, require no temperature tuning, and can be implemented in a few lines of codes. Against other admissible solutions, our estimator is unique and minimizes weight variance; in contrast, prior works use categorical variables or augmented representations to approximate non-categorical variables that induces excess variance and computations. To understand approximation bias for functions beyond the prescribed class, we also derive a non-asymptotic bias bound. In experiments our low order methods match or improve tuned baselines across linear, nonlinear and hierarchical latent-variable models, while out-speeding competitors in every runtime benchmark.

==> sections/1.0_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Discrete latent variables appear in deep generative models, neural sequence
models, and other applications
\citep{def,pvae,second_gsm_poglm}.
For continuous random variables, pathwise gradients are often preferred
because they are unbiased, typically low variance, and compatible with
ordinary backpropagation.
The pathwise identity asks for a weight $w(Z)$ that makes the gradient
exact for every sufficiently regular $f$.
For discrete variables, no such universal weight exists in general.
\lw{In continuous domain: pathwise gradient estimators have nice properties: unbiasedness (exactness), low variance (empirically), cheap}

\lw{Gap: apply pathwise gradient estimators in discrete latent variable optimization.}

Existing estimators navigate the resulting
bias--variance--computation tradeoff using control variates, additional
function evaluations, surrogate derivatives, or continuous relaxations
\citep{mcge_survey,mvd,ste,gsm,concrete}.

\lw{Score/reinforce: unbiased, high variance, needs control variates}
\lw{Measure-value derivative: unbiased but poor scalability with dimensions}
\lw{Categorical: straight-through, relaxations, reinmax -- biased}
\lw{Poisson: relaxed.}
\lw{except reinmax, other methods do not quantify bias.}

\textit{Can we retain the pathwise form while prescribing how much
exactness to preserve?} 
\lw{What does "exactness" mean? I think we need more context to explain the gap in the literature, and what we mean by "controlling how much exactness" -- and why that's a good idea.}

\medskip
\noindent
\begin{minipage}[t]{0.25\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/exactness_full_cropped_v3.png}
\end{minipage}
\hfill
\begin{minipage}[t]{0.35\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/least_norm_trimmed.png}
\end{minipage}
\hfill
\begin{minipage}[t]{0.30\linewidth}
    \vspace{0pt}
    \captionsetup[lstlisting]{font=footnotesize,skip=2pt}
    \begin{lstlisting}[
        style=introcode,
        basicstyle=\ttfamily\fontsize{5.6}{6.2}\selectfont,
        numberstyle=\fontsize{4.8}{5.2}\selectfont,
        numbersep=3pt,
        xleftmargin=0.1em,
        xrightmargin=0.1em,
        caption={Order-2 and order-3 Poisson estimators in pytorch.},
        label={lst:intro-poisson},
        captionpos=t
    ]
...
rate = eta.exp()
z_hard = Poisson(rate).sample()

# order 2:
@w = 0.5 * (z_hard + rate)@
# order 3:
# w = 5*rate/12
#   + (8*rate+1)*z_hard/(12*rate)
#   - z_hard**2/(12*rate)

@z = z_hard + w.detach() * (eta - eta.detach())@
...    \end{lstlisting}
\end{minipage}
\vspace{0.1em}
\captionof{figure}{
Finite-order pathwise \lw{gradient estimator} recipe. \textbf{Left}: we specify order $D$ exactness where $\mathcal{P}_d \subset \mathcal{P}_{d+1}$, while classical pathwise requires exactness for all sufficiently regular $f$. \textbf{Center}: least norm selects the canonical $\mathcal{P}_D$ exact weight, avoiding excess weight variance. \textbf{Right}: the resulting Poisson weights reduce to a few lines of code. \lw{All figure captions and table captions need to be more self-contained. Imagine a reader that directly jumps to figures and results before reading the main text -- what's the key message they can get out of it?}
}
\label{fig:intro-construction}
\medskip

We make the pathwise identity finite-order rather than relaxing or embedding the discrete sample. \lw{what is the pathwise identity? what does finite order mean, and why the form $f'(Z)w_D(Z)$? When explaining these concepts, try to do it at a high-level for introduction.}
We retain estimators of the form $f'(Z)w_D(Z)$, but require exactness only
for $f\in\mathcal P_D$, the polynomials of degree at most $D$.
Choosing $D$ directly prescribes approximation order, but generally leaves
many feasible weights; least-norm selection chooses the canonical one.

\lw{Start with a summarizing sentence. Is this paragraph about the theoretical properties about the gradient estimator?} 
Within $\mathcal P_D$ the gradient identity is exact; outside it and under reasonable regularity conditions, we prove a non-asymptotic bias bound governed by the first unmatched derivative (\ref{prop:smooth-bias}).
Among degree-$D$ exact weights, the least-norm choice uniquely minimizes weight variance (\ref{prop:min-variance}).
Surprisingly, at order 2 the construction exactly recovers the classical
pathwise gradients for scalar location--scale families and Gaussian random
vectors.
At the same order, the categorical formulation also recovers ReinMax,
the most competitive general-purpose categorical gradient estimator
(\secref{sec:order2-connections}). \lw{Conclude with why these are interesting properties.} 

As shown in \secref{sec:method}, solving for the canonical weights reduces estimator design to a one-time $D\times D$ linear solve involving only moments of the target law and their parameter derivatives.
For the orders used in our paper, this is only a 2 by 2 or 3 by 3 solve, followed by affine or quadratic evaluation independent of support size.
The resulting estimator preserves the exact forward sample and requires only one downstream forward--backward pass, with no temperature tuning or continuous relaxation.
For Poisson, the resulting weights reduce to a few lines of PyTorch
(Listing~\ref{lst:intro-poisson}).


% \paragraph{Contributions:}
% \begin{itemize}[leftmargin=*, itemsep=1pt, topsep=2pt]

% \item
% We extend pathwise gradients to discrete random variables: the pathwise identity nails down the gradient form, degree-$D$ exactness prescribes approximation order, and least-norm selection chooses a weight within each exactness class (\secref{sec:method}).

% \item
% For common discrete laws, the solved estimator has polynomial weights that are simple to implement and whose fixed-order evaluation is independent of support size (\secref{sec:pois-example}, \secref{app:estimators}, \secref{sec:two-parameter-st}).

% \item
% We prove that the least-norm weight is unique and minimizes weight variance within each exactness class, derive a non-asymptotic bias bound for smooth downstream functions, and decompose excess variance into auxiliary-variable noise and orthogonal null components (\secref{sec:theory}).

% \item
% Across neural sequence models, nonlinear VAEs, and hierarchical topic models, the estimator family is competitive with or outperforms tuned baselines; orders 2 and 3 rank first and second in every runtime benchmark (\secref{sec:experiments}).

% \end{itemize}

\paragraph{Contributions:}
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=2pt]

\item
\textbf{Finite-order discrete pathwise gradients:}
We replace classical pathwise exactness by $\mathcal{P}_D$ exactness, yielding order-indexed pathwise gradient approximations for hard discrete samples (\secref{sec:method}).

\item
\textbf{Generality across discrete laws:}
For common discrete laws, the same moment-based recipe yields closed-form polynomial weights from a small linear system.
The resulting estimators are simple to implement and their evaluation cost is independent of support size
(\secref{sec:method}, \appref{app:estimators},
\secref{sec:two-parameter-st}).

\item
\textbf{Canonical solution and error theory:}
Least-norm selection gives the unique minimum-weight-variance solution within each exactness class.
We derive a non-asymptotic bias bound outside the matched polynomial class and characterize excess variance introduced by categorical and compound reductions (\secref{sec:theory}).

\item
\textbf{Specialist-level empirical performance:} Across neural sequence models, nonlinear VAEs, and hierarchical topic models, the estimator family matches or outperforms tuned baselines; orders 2 and 3 rank first and second in every runtime benchmark (\secref{sec:experiments}).


\end{itemize}

==> sections/3.05_table_of_connections.tex <==

\begin{table*}[t]
\centering
\caption{Correspondence between numerical and probabilistic concepts, will probably move it to appendix later/journal/use for presentation.}
\label{tab:numerical_probabilistic_correspondence}
\small
\begin{threeparttable}
\begin{tabular}{@{}p{0.20\textwidth} p{0.22\textwidth} p{0.52\textwidth}@{}}
\toprule
\textbf{Numerical Math}
&
\textbf{Probabilistic Modeling}
&
\textbf{The connections}
\\
\midrule

Exactness
&
Unbiasedness
&
Under linearity, polynomial exactness $\leftrightarrow$ monomial exactness; exactness under expectation $\leftrightarrow$ unbiasedness.
\\[0.6em]

Monomial constraints
&
Moment-derivative constraints
&
Testing the weights on $f(z)=z^d$ requires it to reproduce the moment derivatives
$\partial_\theta \mathbb{E}_\theta[Z^d]$.
Monomials are the test functions; moments are their expectations.
\\[0.6em]

Approximation error
&
Bias
&
In numerical quadrature, the residual term from modeling polynomials
The discrepancy between the expected rule and the target derivative is the estimator's bias.
\\[0.6em]

Minimum/Least norm
&
Minimum weight variance
&
The Hilbert space norm is $\mathbb{E}_\theta[w^2]$.
And as a preview to our theory section, the first constraint actually fixes $\mathbb{E}_\theta[w]$ for any admissible $w$, which means minimizing weight norm and minimizing weight variance are equivalent.
\\[0.6em]

Gram matrix
&
Raw Second-order moment matrix
&
This one is self explanatory
\\[0.6em]

Orthogonality
&
Un-correlations (when centered)
&
We actually recover many named orthogonal polynomials that researchers developed for certain distributions. For example, for Poisson, we recovered Charlier polynomials.
\\[0.6em]

% Orthogonal projection onto a feature span
% &
% Population least-squares regression
% &
% Projecting a weight onto polynomial features gives its best mean-square linear prediction from those features.
% The discarded component is the regression residual.
% This is not generally conditional expectation, which projects onto all square-integrable functions of the conditioning variable.
% \\

\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}


==> sections/3.0_method.tex <==

\section{Our Proposed Discrete Pathwise Extension}
% \label{sec:method}
\lw{Let's create a name for the proposed method}

\lw{Add a preamble for the method section, e.g. "What is the problem. We first prescribe the general recipe. Then give an example. Then Discuss ... }


For a prescribed order $D\geq 1$, let $\mathcal P_D$ denote the
polynomials of degree at most $D$.
We seek an estimator 
\begin{equation}
\widehat g_D
=
w_D(Z)f'(Z),
\qquad
\E_\theta[w_D(Z)f'(Z)]
=
\partial_\theta\E_\theta[f(Z)]
\quad
\text{for every }f\in\mathcal P_D,
\label{eq:finite-order-pathwise1}
\end{equation}

\lw{While $\hat g_D$ is defined, has it been used afterwards?}

Equip $L^2(p_\theta)$ with
$\langle u,v\rangle_\theta=\E_\theta[u(Z)v(Z)]$.
Testing \eqref{eq:finite-order-pathwise} on $\{f(z)=z^d, 
\}_{d=1}^D$ \lw{Fix the extra $','$. In addition, it's a good practice to add a descriptive phrase before a math term, e.g. "Testing (2) on the polynomial test functions up to order $D$ ...".}

\lw{On a separate note, I'd recommend using the `cleverref` package to handle all references (equations, figures, sections, tables,...)}

yields $D$ linear moment constraints, since the monomials span $\mathcal P_D$.
These constraints underspecify the weight, so we resolve the ambiguity by selecting the least-norm solution \lw{this is only an issue when $D > K?$ where $K$ is the support of the discrete distribution?} \lw{And explain why using least norm not others for resolving under-determination?}:
\begin{equation}
\begin{aligned}
&
\operatorname*{arg\,min}_{w_D\in L^2(p_\theta)}
\|w_D\|_2
\\
\text{s.t.}\qquad
\langle w_D,Z^{d-1}\rangle_\theta
&=
\frac1d\partial_\theta\E_\theta[Z^d],
\qquad
d=1,\ldots,D.
\end{aligned}
% \label{eq:min-norm-moment-problem1}
\end{equation}

\lw{Let's be slow in derivation. Start from the high-level idea of solving this optimization problem. E.g. why does $w$ takes the form of polynomials? }
Writing
$v_D(z)=(1,z,\ldots,z^{D-1})^\top$
and collecting the right-hand sides in $b_D$. 
The constraint functionals have monomial Riesz representers whose span is $V_D=\operatorname{span}\{1,Z,\ldots,Z^{D-1}\}$.
Components orthogonal to $V_D$ do not affect feasibility, so the
least-norm solution lies in $V_D$.
Whenever $G_D$ is nonsingular
(Proposition~\ref{prop:min-norm-solution}),
\begin{equation}
\boxed{
G_D
=
\E_\theta[v_D(Z)v_D(Z)^\top],
\qquad
w_D^\star(z)
=
v_D(z)^\top G_D^{-1}b_D.
}
\label{eq:gram-solution1}
\end{equation}

Each target law enters only through its moments and their parameter
derivatives.
The recipe is mechanical: 
\lw{Organize it into a numbered list or a pseudo-algorithm fashion.} 
compute moments through order $2D-2$ to form
$G_D$, differentiate the first $D$ moments to form $b_D$, and solve the
$D\times D$ system $G_Dc_D=b_D$.
For the estimators used in the main experiments, the $2\times2$ and
$3\times3$ systems are solved once in closed form; runtime evaluation then
amounts only to an affine or quadratic polynomial.

\lw{Add some remarks on the hidden assumptions and implications. E.g. The expectation on the RHS of (3) needs to be tractable, which is essentially a requirement on the discrete distribution class -- for what discrete distributions, is this tractable and the method applies? It'd also be nice to have a discussion on the choice of $D$.}

The solution also has an orthogonal-polynomial interpretation.
If $G_D=L_DL_D^\top$ is the Cholesky factorization, then
$q_D=L_D^{-1}v_D$ satisfies
$\E_\theta[q_D(Z)q_D(Z)^\top]=I_D$.
Therefore $L_D^{-1}b_D$ gives the coordinates of $w_D^\star$ in the
distribution's orthonormal polynomial basis.
Polynomial exactness and norm-minimal differentiation formulas are
classical in numerical analysis \citep{gautschi2012}, and minimum-norm
selection under linear constraints is standard \citep{boyd2004}.  \lw{Why is this interesting and what are the practical relavences? Is it connected to bias-variance tradeoffs?}

Proposition~\ref{prop:min-variance} shows that the resulting weight is also the unique minimum-weight-variance solution. \lw{Why mentioning Prop 4.1 here? What's the connection to the prior part?}


\appref{app:estimators} gives additional closed-form weights for common discrete laws, and \appref{sec:two-parameter-st} extends the implementation to multiple parameter coordinates.


\subsection{Example: Poisson distribution}
% \label{sec:pois-example}

Let $Z\sim\operatorname{Pois}(\lambda)$ with $\eta=\log\lambda$.
Substituting the standard Poisson moments into
\eqref{eq:gram-solution} gives
\begin{equation}
\boxed{
w_2^\star(Z)
=
\frac{Z+\lambda}{2},
\qquad
w_3^\star(Z)
=
\frac{5\lambda}{12}
+
\frac{8\lambda+1}{12\lambda}Z
-
\frac{1}{12\lambda}Z^2.
}
% \label{eq:poisson-weights}
\end{equation}

These are the Poisson weights in Listing~\ref{lst:intro-poisson}.
The mathematical estimator is
$\widehat g_D=w_D^\star(Z)f'(Z)$. 
In the implementation, stop-gradient sets the autodiff derivative
$\partial Z/\partial\eta$ to $w_D^\star(Z_{\mathrm{hard}})$ while leaving
the forward value equal to $Z_{\mathrm{hard}}$.

\paragraph{Weak-derivative interpretation.}
The same weights also follow from the difference identity
\[
\partial_\eta\E[f(Z)]
=
\lambda\E[f(Z+1)-f(Z)]
=
\lambda\E\!\left[\int_0^1 f'(Z+t)\,dt\right].
\]
Applying interpolatory quadrature to the integral sets the exactness order.
The Poisson shift identities
$\lambda\E[g(Z+1)]=\E[Zg(Z)]$
and
$\lambda^2\E[g(Z+2)]=\E[Z(Z-1)g(Z)]$
then rewrite the neighboring-state derivatives as expectations under the
original sample, yielding the same weights.
The two-node rule recovers order 2, while the three-node recovers order 3;
\appref{app:mvd-quadrature} gives the algebraic proof.

\subsection{Order-2 Connections}
\label{sec:order2-connections}

\paragraph{Continuous pathwise recoveries.}
At order 2, the construction is fully exact for scalar location--scale
families and Gaussian random vectors.
For a scalar location--scale family
$Z=\mu_\theta+\sigma_\theta\epsilon$,
it gives
$w_2^\star(Z)=\partial_\theta Z$.
The analogous vector construction for
$Z\sim\mathcal N(\mu_\theta,\Sigma_\theta)$
gives
$W_2^\star(z)=\dot\mu_\theta+A(z-\mu_\theta)$,
where dots denote differentiation with respect to the parameter coordinate
and $A=A^\top$ solves
$A\Sigma_\theta+\Sigma_\theta A=\dot\Sigma_\theta$.
This is the minimum-kinetic-energy Gaussian pathwise field of
\citet{jankowiak2018pathwise}.
Formal statements and proofs appear in \appref{app:pathwise}.

\paragraph{Categorical straight-through \lw{and ReinMax?} connections.}
A finite scalar law on support
$x=(x_1,\ldots,x_K)^\top$
can be represented by
$C\sim\operatorname{Cat}(p)$
and
$Z=x^\top C$; unbounded laws require truncation.
ReinMax is a categorical straight-through estimator derived as a
second-order correction to ST \citep{reinmax}, which empirically outperforms other etimator on a multitude of benchmarks.
Under our separate polynomial criterion,
\appref{app:categorical-connections} proves that its $\tau=1$ weight is
degree-2 exact.
The same appendix shows that categorical least-norm selection recovers the
$\tau\to\infty$ one-hot MVE of \citet{hooperetal2026}, while the scalar
degree-2 construction recovers their hard 1D MVE.
These results place ReinMax and both MVE correspondences inside the same
degree-2 exactness framework; Section~\ref{sec:theory} then analyzes the
scalar Poisson weight induced by categorical ReinMax.


==> sections/3.0_method_old.tex <==
\section{A General Recipe of Extending Pathwise Gradients}
\label{sec:method}

We seek a discrete gradient estimator with three properties:

\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=2pt]

    \item \textbf{Pathwise Chain-rule form:}
    for $Z\sim p_\theta$ and differentiable $f$,
    $\hat{g}_D=w_D(Z)f'(Z)$.

    \item \textbf{Degree-$D$ exactness:}
    $\mathbb E_\theta[w_D(Z)f'(Z)]
    =\partial_\theta\mathbb E_\theta[f(Z)]$
    for every $f\in\mathcal P_D$.

    \item \textbf{Least-$L^2$-norm selection:}
    among degree-$D$ exact weights, choose
    $w_D^\star\in\operatorname*{arg\,min}_w\mathbb E_\theta[w(Z)^2]$.

\end{itemize}

Equip $L^2(p_\theta)$ with
$\langle u,v\rangle_\theta=\mathbb E_\theta[u(Z)v(Z)]$.
Degree-$D$ exactness imposes $D$ linear constraints but generally leaves infinitely many feasible weights.
We select the least-norm solution:
\begin{equation}
\begin{aligned}
&
\operatorname*{arg\,min}_{w_D\in L^2(p_\theta)}
\|w_D\|_2
\\
\text{s.t.}\qquad
\langle w_D,Z^{d-1}\rangle_\theta
&=
\frac1d\partial_\theta\mathbb E_\theta[Z^d],
\qquad d=1,\ldots,D.
\end{aligned}
\label{eq:min-norm-moment-problem}
\end{equation}
Writing $v_D(z)=(1,z,\ldots,z^{D-1})^\top$ and collecting the right-hand sides in $b_D$, the Riesz representers of the constraints are $1,Z,\ldots,Z^{D-1}$.
Hence the least-norm solution lies in
$V_D=\operatorname{span}\{1,Z,\ldots,Z^{D-1}\}$.
Whenever $G_D$ is nonsingular (Proposition~\ref{prop:min-norm-solution}),
\begin{equation}
    \boxed{
        G_D=\mathbb E_\theta[v_D(Z)v_D(Z)^\top],
        \qquad
        w_D^\star(z)=v_D(z)^\top G_D^{-1}b_D .
    }
    \label{eq:gram-solution}
\end{equation}

Thus order $D$ produces a degree-$(D-1)$ polynomial weight from a $D\times D$ moment system.
For the closed-form estimators used here, solving the system is a one-time design cost.
The first exactness constraint fixes $\E_\theta[w_D(Z)]$, so the least-norm solution also uniquely minimizes weight variance within its exactness class.
If $G_D=L_DL_D^\top$ is the Cholesky factorization, then $q_D=L_D^{-1}v_D$ satisfies $\mathbb E_\theta[q_D(Z)q_D(Z)^\top]=I_D$.
Therefore $L_D^{-1}b_D$ gives the coordinates of the variance-optimal weight in the distribution's orthonormal polynomial basis.

Polynomial exactness and norm-minimal differentiation formulas are classical in numerical analysis \citep{gautschi2012}, and minimum-norm selection under linear constraints is standard \citep{boyd2004}.
Here the constraints encode parameter derivatives of distributional moments; because exactness fixes the mean, minimizing the $L^2(p_\theta)$ norm also minimizes weight variance within the class.
Appendix~\ref{app:estimators} gives additional closed-form weights for common discrete laws, and Appendix~\ref{sec:two-parameter-st} extends the implementation to multiple parameter coordinates.

\subsection{Example: Poisson distribution}
\label{sec:pois-example}
Let $Z\sim\operatorname{Pois}(\lambda)$ with $\eta=\log\lambda$.
The order-3 Gram matrix and constraint vector are
\begin{equation}
    G_3=
    \begin{pmatrix}
        1
        & \lambda
        & \lambda^2+\lambda
        \\
        \lambda
        & \lambda^2+\lambda
        & \lambda^3+3\lambda^2+\lambda
        \\
        \lambda^2+\lambda
        & \lambda^3+3\lambda^2+\lambda
        & \lambda^4+6\lambda^3+7\lambda^2+\lambda
    \end{pmatrix},
    \qquad
    b_3=
    \begin{pmatrix}
        \lambda\\
        \lambda^2+\lambda/2\\
        \lambda^3+2\lambda^2+\lambda/3
    \end{pmatrix}.
    \label{eq:poisson-gram}
\end{equation}
The order-2 system uses the leading $2\times2$ block of $G_3$ and the first two entries of $b_3$.
For $v_2(z)=(1,z)^\top$ and $v_3(z)=(1,z,z^2)^\top$, solving the two systems gives
\begin{equation}
    G_2^{-1}b_2
    =
    \begin{pmatrix}
        \lambda/2\\[1mm]
        1/2
    \end{pmatrix},
    \qquad
    G_3^{-1}b_3
    =
    \begin{pmatrix}
        5\lambda/12\\[1mm]
        (8\lambda+1)/(12\lambda)\\[1mm]
        -1/(12\lambda)
    \end{pmatrix}.
    \label{eq:poisson-coefficients}
\end{equation}
Substitution into $w_D^\star(z)=v_D(z)^\top G_D^{-1}b_D$ yields
\begin{equation}
    \boxed{
        w_2^\star(Z)=\frac{Z+\lambda}{2},
        \qquad
        w_3^\star(Z)
        =
        \frac{5\lambda}{12}
        +\frac{8\lambda+1}{12\lambda}Z
        -\frac{1}{12\lambda}Z^2
    }
    \label{eq:poisson-weights}
\end{equation}
These are the Poisson estimators shown in Listing~\ref{lst:intro-poisson}.
The construction extends to any prescribed order; Appendix~\ref{app:estimators}, for example, gives the cubic order-4 weight.
Under the log-rate parameterization, the order-4 weight variance diverges as $\lambda\downarrow0$, illustrating the variance cost of higher exactness.

\paragraph{Poisson MVD and quadrature.}
The same weights also admit a weak-derivative interpretation:
\[
\partial_\eta\E[f(Z)]
=
\lambda\E[f(Z+1)-f(Z)]
=
\lambda\E\!\left[\int_0^1 f'(Z+t)\,dt\right].
\]
Interpolatory quadrature sets the approximation order, while the Poisson shift identities $\lambda\E[g(Z+1)]=\E[Zg(Z)]$ and $\lambda^2\E[g(Z+2)]=\E[Z(Z-1)g(Z)]$ return neighboring-state derivatives to the law of the original sample, yielding a same-path weight.
The two-node rule at $t=0,1$ recovers order 2, and the three-node rule at $t=0,1,2$ recovers order 3; Appendix~\ref{app:mvd-quadrature} gives the algebra.

\subsection{Order-2 recoveries}
The same construction is fully exact in classical continuous families.

\begin{proposition}[Pathwise recoveries]
\label{prop:pathwise-recoveries}
\textup{(a)} \textbf{Scalar location--scale families.}
Let $Z=\mu_\theta+\sigma_\theta\varepsilon$, where $\sigma_\theta>0$ and $\varepsilon$ is independent of $\theta$ with mean zero and unit variance.
Then $w_2^\star(Z)=\partial_\theta Z$, so the estimator is exact for every sufficiently regular $f$.

\smallskip
\textup{(b)} \textbf{Gaussian random vectors.}
Let $Z\sim\mathcal N(\mu_\theta,\Sigma_\theta)$ with $\Sigma_\theta\succ0$, and let dots denote derivatives with respect to the scalar parameter $\theta$.
For estimators $\widehat g=W(Z)^\top\nabla f(Z)$, the quadratic-exact least-norm field is
\begin{equation}
W_2^\star(z)
=
\dot\mu+A(z-\mu_\theta),
\qquad
A=A^\top,
\qquad
A\Sigma_\theta+\Sigma_\theta A=\dot\Sigma,
\label{eq:gaussian-vector-weight}
\end{equation}
and is exact for every sufficiently regular $f$.
\end{proposition}

Proofs appear in Appendix~\ref{app:pathwise}.
Thus order 2 recovers exact pathwise differentiation in both settings; for Gaussian vectors, it recovers the minimum-kinetic-energy pathwise field of \citet{jankowiak2018pathwise}.
The framework also recovers the hard 1D MVE for integer categoricals at order 2, while higher orders continue beyond these order-2 correspondences (Appendix~\ref{app:connections}).


==> sections/4.0_theory.tex <==
\section{Theory}
\label{sec:theory}

\lw{The current section feels a bit crowded. I suggest to keep the main results with even informal statements in the main text; You can say ``all the formal statement and proofs are provided in Appendix xx". For example, Prop 4.3 could show the variance decomposition without displaying the 3-term weight decomposition. Corollary 4.4 could foreground the $\lambda^2$ gap... Also, after each statement, immediately start one sentence takeaway in plain language. And then  explain in details, if necessary.}
\donghan{sorry i haven't been able to fully renovate this section into what you want. can we do one example in sync, then i can work on it.}

Having defined the finite-order recipe, we establish the solution's uniqueness \lw{Clarify canonicality} as well as weight-variance optimality, bound its bias outside $\mathcal P_D$ \lw{I would typically write a short description before math notation, like ``degree-D function class $\mathcal P_D$ for better readability}\donghan{given we earlier defined $P_D$, i think this should be resolved now}, and decompose the excess weight
variance introduced by non-native representations.
%We then make the variance geometry concrete for Poisson ReinMax and the Gamma--Poisson representation.
We illustrate these results by quantifying the excess weight variance of categorical ReinMax applied to Poisson variables and of a Gamma--Poisson representation of Negative-Binomial variables. 

1. write intuitively what the proposition is going to do before the proposition
2. after proposition, we write intuitively how the argument goes.

In the proposition below, we show that any order $D$ solution to  \cref{eq:min-norm-moment-problem} is unique, and weight-variance is optimal. 

\begin{proposition}
\label{prop:min-variance}
Let
$V_D=\operatorname{span}\{1,Z,\ldots,Z^{D-1}\}$,
and assume that $G_D$ is nonsingular.
Every degree-$D$ exact weight $w\in L^2(p_\theta)$ admits a unique
decomposition
\begin{equation}
\begin{aligned}
w
&=
w_D^\star+r,
\qquad
r\perp V_D;
\qquad
\operatorname{Var}_\theta[w(Z)]
=
\operatorname{Var}_\theta[w_D^\star(Z)]+\|r\|_2^2.
\end{aligned}
\label{eq:min-variance-gap}
\end{equation}
Consequently, $w_D^\star$ uniquely minimizes both the $L^2(p_\theta)$
norm and weight variance within the degree-$D$ exact class.
\end{proposition}
% Exactness fixes the projection onto $V_D$; any remaining component is
% invisible to the prescribed constraints and contributes $\|r\|_2^2$ to
% both the squared norm and weight variance.
Intuitively, the argument is any order $D$ solution must decompose into a base component and a null component. The base component is precisely our solution; the null component lives in the kernel space of the constraints in \cref{eq:min-norm-moment-problem}, so it will not disturb the unbiasedness of our solution; however, it does add excess weight variance.

In proposition below, we characterize the smooth-function bias bound of our method beyond prescribed exactness class.
\begin{proposition}[]
\label{prop:smooth-bias}
For a degree-$D$ exact weight $w$, define
\[
B_w(f)
=
\E_\theta[w(Z)f'(Z)]
-
\partial_\theta\E_\theta[f(Z)].
\]
Fix $a\in\mathbb R$ independently of $\theta$, let
$s_\theta(Z)=\partial_\theta\log p_\theta(Z)$, and write
$m_k(a)=\E_\theta[|Z-a|^k]$.
Assume that the score identity holds for $f$ and every
$h\in\mathcal P_D$, that $w,s_\theta\in L^2(p_\theta)$,
that $m_{2D+2}(a)<\infty$, and that
$f\in C^{D+1}(\mathbb R)$ with
$\|f^{(D+1)}\|_\infty<\infty$.
Then
\begin{equation}
|B_w(f)|
\le
\|f^{(D+1)}\|_\infty
\left[
\frac{m_{2D}(a)^{1/2}}{D!}\|w\|_2
+
\frac{m_{2D+2}(a)^{1/2}}{(D+1)!}\|s_\theta\|_2
\right].
\label{eq:smooth-bias-bound}
\end{equation}
\end{proposition}

Degree-$D$ exactness cancels the degree-$D$ Taylor polynomial, so the
remaining bias is controlled by the first unmatched derivative
$f^{(D+1)}$, moments of the law, and the score norm.
Among degree-$D$ exact weights, $w_D^\star$ minimizes the bound's only
weight-dependent term.
\donghan{add also why modern NNs will work with our theorem}

\begin{proposition}[Rao--Blackwellization and native projection]
\label{prop:rao-blackwell}
Suppose that $p_\theta(z,u)$ is an augmented representation of the marginal
law $p_\theta(z)$, and let
$\widetilde w_D(U,Z)\in L^2$ be degree-$D$ exact under the joint law.
Define
$\bar w_D(Z)=\E_\theta[\widetilde w_D(U,Z)\mid Z]$.
Then $\bar w_D$ is degree-$D$ exact and
\begin{equation}
\widetilde w_D
=
w_D^\star
+
(\bar w_D-w_D^\star)
+
(\widetilde w_D-\bar w_D),
\label{eq:rao-blackwell-orthogonal-decomposition}
\end{equation}
where the three terms are mutually orthogonal.
Consequently,
\begin{equation}
\operatorname{Var}_\theta[\widetilde w_D]
=
\operatorname{Var}_\theta[w_D^\star]
+
\E_\theta\!\left[
\operatorname{Var}_\theta(\widetilde w_D\mid Z)
\right]
+
\|\bar w_D-w_D^\star\|_2^2.
\label{eq:rao-blackwell-decomposition}
\end{equation}
\end{proposition}

The conditional-variance term is auxiliary-variable noise removed by
Rao--Blackwellization.
The final term survives conditioning and is removed only by native
least-norm projection.
Thus Rao--Blackwellization is sufficient exactly when
$\bar w_D=w_D^\star$; in all cases, the native weight has no greater
variance than either the augmented weight or its Rao--Blackwellization.

The $\tau=1$ ReinMax weight characterized is degree-2 exact .
\lw{Resolve the reference error}\donghan{rephrased, please review}
When applying the $\tau=1$ ReinMax to Poisson, the order 2 exactness of ReinMax is inherited.
Proposition~\ref{prop:min-variance} therefore identifies its orthogonal
excess component in the large-truncation Poisson limit.

\begin{corollary}[Poisson ReinMax null component]
\label{prop:poisson-reinmax}
Let $Z\sim\operatorname{Pois}(\lambda)$ under the log-rate parameterization
$\eta=\log\lambda$.
\lw{Could we specify the renormalized categorical truncation and explain why $\tau=1$ is singled out?}
\donghan{sorry what do you mean? t=1 needs to be singled out because at non-one t, reinmax is not second order.}
At $\tau=1$, the large-truncation limit of categorical ReinMax has weight
\begin{equation}
\begin{aligned}
w_{\mathrm{RM}}(Z)
&=
\frac{\lambda+(Z-\lambda)^2}{2}
\\
&=
\underbrace{\frac{Z+\lambda}{2}}_{w_2^\star(Z)}
+
\underbrace{
\frac{(Z-\lambda)^2-(Z-\lambda)-\lambda}{2}
}_{r_{\mathrm{RM}}(Z) \perp V_2},
\\
\operatorname{Var}[w_{\mathrm{RM}}(Z)]
&
=
\operatorname{Var}[w_2^\star(Z)]
+
\frac{\lambda^2}{2}.
\end{aligned}
\label{eq:poisson-reinmax-decomposition}
\end{equation}
\end{corollary}

Thus the large-truncation Poisson ReinMax weight remains degree-2 exact
but is nonminimal; its orthogonal residual adds $\lambda^2/2$ to the
weight variance.
\lw{Emphasize this is a weight-variance gap, not a universal gradient-variance gap?}

We next apply Proposition~\ref{prop:rao-blackwell} to the Gamma--Poisson
representation, which reuses a Poisson estimator for a Negative-Binomial
law through an auxiliary rate.
\begin{corollary}[Gamma--Poisson representation at orders 2 and 3]
\label{cor:gamma-poisson}
Let
\[
\Lambda
\sim
\operatorname{Gamma}\!\left(
r,\operatorname{rate}=\frac{1-p}{p}
\right),
\qquad
Z\mid\Lambda\sim\operatorname{Pois}(\Lambda),
\qquad
\eta=\operatorname{logit}p,
\]
and let $\widetilde w_D(Z,\Lambda)$ be the compound estimator obtained by
applying the order-$D$ Poisson weight conditionally on $\Lambda$.
\lw{Could we state the Negative-Binomial marginal law and explain why this parameterization permits the conditional Poisson weight?}
\donghan{sorry what do you mean? im just expanding out what the weight would algebraically be, if we apply order 2 (3) poisson weight to poisson + gamma}
With
$\bar w_D(Z)=\E[\widetilde w_D(Z,\Lambda)\mid Z]$,
\begin{equation}
\begin{aligned}
\bar w_2
&=
w_2^\star,
\\
\bar w_3
&=
w_3^\star+r_3,
\qquad
r_3\perp V_3,
\qquad
r_3\not\equiv0.
\end{aligned}
\label{eq:gamma-poisson-conditioning}
\end{equation}
\lw{Could we briefly explain why $r_3$ is nonzero or point to the appendix argument comparing tail growth?}
\donghan{intuitively, this is due to order 3 weights are not linear anymore.}
Consequently,
\begin{equation}
\begin{aligned}
\operatorname{Var}[\widetilde w_2]
&=
\operatorname{Var}[w_2^\star]
+
\E\!\left[
\operatorname{Var}(\widetilde w_2\mid Z)
\right],
\\
\operatorname{Var}[\widetilde w_3]
&=
\operatorname{Var}[w_3^\star]
+
\E\!\left[
\operatorname{Var}(\widetilde w_3\mid Z)
\right]
+
\|r_3\|_2^2.
\end{aligned}
\label{eq:gamma-poisson-variance}
\end{equation}
\end{corollary}

At order 2, Rao--Blackwellization closes the gap: the Rao--Blackwellized
compound estimator coincides with the native Negative-Binomial estimator,
so all excess weight variance comes from the auxiliary Gamma variable.
At order 3, it does not: conditioning removes the auxiliary noise but
leaves a nonminimal $Z$-only component, so native least-norm projection
yields a further reduction in weight variance.
The two orders therefore separate variance removed by conditioning from
variance that survives it.


==> sections/4.0_theory_old.tex <==
\section{Optimality and Approximation Properties}
\label{sec:theory}

We first establish two general consequences of the construction: the least-norm weight uniquely minimizes weight variance within its exactness class, and degree-$D$ exactness gives a non-asymptotic bias bound for smooth downstream functions.
We then illustrate the null-space interpretation by decomposing Poisson ReinMax under categorical embedding at $\tau=1$.
Proofs appear in Appendix~\ref{app:proofs}.

\subsection{Uniqueness and weight-variance optimality}
\label{sec:minimum-norm}

\begin{proposition}[Null-space decomposition and optimality]
\label{prop:min-variance}
Let $V_D=\operatorname{span}\{1,Z,\ldots,Z^{D-1}\}$ and assume $G_D$ is nonsingular.
Every degree-$D$ exact weight $w\in L^2(p_\theta)$ has the unique decomposition
\begin{equation}
w=w_D^\star+r,
\qquad
r\perp V_D,
\label{eq:exact-weight-decomposition}
\end{equation}
and satisfies
\begin{equation}
\mathbb E_\theta[w(Z)^2]
=
b_D^\top G_D^{-1}b_D
+
\mathbb E_\theta[r(Z)^2].
\label{eq:min-norm-gap}
\end{equation}
Consequently, $w_D^\star$ is the unique least-norm degree-$D$ exact weight.
Moreover,
\begin{equation}
\operatorname{Var}_\theta[w(Z)]
=
\operatorname{Var}_\theta[w_D^\star(Z)]
+
\mathbb E_\theta[r(Z)^2],
\label{eq:min-variance-gap}
\end{equation}
so $w_D^\star$ also uniquely minimizes weight variance within the class.
\end{proposition}

Degree-$D$ exactness fixes the weight's projection onto $V_D$.
Any remaining component is invisible to the prescribed test functions but increases both the raw second moment and weight variance; the least-norm choice removes exactly this null component.
Because the degree-$(D+1)$ exactness class is contained in the degree-$D$ class, Proposition~\ref{prop:min-variance} shows that $\lVert w_D^\star\rVert_2^2$ and $\operatorname{Var}_\theta[w_D^\star(Z)]$ are nondecreasing in $D$ whenever the corresponding Gram matrices are nonsingular.

For the gradient estimator, whenever $\|f'\|_\infty<\infty$,
\begin{equation}
\operatorname{Var}_\theta[w(Z)f'(Z)]
\le
\E_\theta[w(Z)^2f'(Z)^2]
\le
\|f'\|_\infty^2\|w\|_2^2.
\label{eq:gradient-variance-bound}
\end{equation}
Thus the least-norm choice minimizes this uniform upper bound within each exactness class, while the exact estimator variance can still depend on the interaction between $w$ and $f'$.

\subsection{Bias beyond polynomial exactness}
\label{sec:bias}

Polynomial exactness also controls bias beyond the matched polynomial class.

\begin{proposition}[Smooth-function bias bound]
\label{prop:smooth-bias}
For any degree-$D$ exact weight $w$, define
\[
B_w(f)
=
\mathbb E_\theta[w(Z)f'(Z)]
-
\partial_\theta\mathbb E_\theta[f(Z)].
\]
Fix $a\in\mathbb R$ independent of $\theta$.
Assume the score identity $\partial_\theta\mathbb E_\theta[h(Z)]=\mathbb E_\theta[s_\theta(Z)h(Z)]$ holds both for $h=f$ and for every $h\in\mathcal P_D$, where $s_\theta(Z)=\partial_\theta\log p_\theta(Z)$.
Suppose $w,s_\theta\in L^2(p_\theta)$, $\mathbb E_\theta[|Z-a|^{2D+2}]<\infty$, and $f\in C^{D+1}(\mathbb R)$ with $\|f^{(D+1)}\|_\infty<\infty$.
Then
\[
|B_w(f)|
\le
\|f^{(D+1)}\|_\infty
\left[
C_{D,w}(a)\|w\|_2
+
C_{D,s}(a)\|s_\theta\|_2
\right],
\]
where $C_{D,w}(a)$ and $C_{D,s}(a)$ depend only on $D$ and moments of $p_\theta$ around $a$; Appendix~\ref{app:bias-proof} gives their explicit forms.
\end{proposition}

Thus degree-$D$ exactness controls smooth-function bias through the first unmatched derivative, $f^{(D+1)}$, and moments of the law.
Among degree-$D$ exact weights, the least-norm weight minimizes the weight-dependent term.

\subsection{Application: null-space component in Poisson ReinMax}
\label{sec:reinmax-big-var}

We apply the null-space decomposition to compare the native Poisson order-2 weight with the categorical ReinMax limit at $\tau=1$.

\begin{corollary}[Null-space component in Poisson ReinMax]
\label{prop:poisson-reinmax}
Let $Z\sim\operatorname{Pois}(\lambda)$ under the log-rate parameterization $\eta=\log\lambda$.
At $\tau=1$, the limit of ReinMax over increasingly large categorical truncations has weight
\begin{equation}
\begin{aligned}
w_{\mathrm{RM}}(Z)
&=
\frac{\lambda+(Z-\lambda)^2}{2}
=
\underbrace{\frac{Z+\lambda}{2}}_{w_2^\star(Z)}
+
\underbrace{
\frac{(Z-\lambda)^2-(Z-\lambda)-\lambda}{2}
}_{r_{\mathrm{RM}}(Z)}, \\
r_{\mathrm{RM}}
&\perp\operatorname{span}\{1,Z\},
\qquad
\lVert r_{\mathrm{RM}}\rVert_2^2
=
\frac{\lambda^2}{2}.
\end{aligned}
\label{eq:poisson-reinmax-decomposition}
\end{equation}
Consequently,
\begin{equation}
\operatorname{Var}[w_{\mathrm{RM}}(Z)]
=
\operatorname{Var}[w_2^\star(Z)]
+
\frac{\lambda^2}{2},
\qquad
\lVert w_{\mathrm{RM}}\rVert_2^2
=
\lVert w_2^\star\rVert_2^2
+
\frac{\lambda^2}{2}.
\label{eq:poisson-reinmax-gap}
\end{equation}
\end{corollary}

Because the residual is orthogonal to the quadratic exactness span, adding it preserves quadratic exactness but adds $\lambda^2/2$ to both the raw second moment and weight variance.
Outside the quadratic class, the estimators differ by $\E[r_{\mathrm{RM}}(Z)f'(Z)]$, which need not vanish.
The bound in Proposition~\ref{prop:smooth-bias} therefore has a larger weight-dependent term for ReinMax.
Appendices~\ref{app:reinmax-nef} and~\ref{app:reinmax-poisson} give the proof.


==> sections/5.0_experiments.tex <==
\section{Numerical Experiments}
\label{sec:experiments}
We test four empirical claims: 
(i) Fini is unbiased for functions inside its prescribed unbiasedness class; 
(ii) For Poisson, Fini at low-order match or outperform competitors on nonlinear and hierarchical scenarios beyond their prescribed unbiasedness class;
(iii) the same construction performs well for other common discrete variables such as Negative Binomial and Binomial;
and (iv) among different types of GPU and benchmarks, our low-order estimators consistently outspeed all competitors. 

%Among different types of GPU and benchmarks, our low-order estimators consistently outspeed all competitors. 

Our main Poisson-specific comparator is EAT-cubic, which differentiates a relaxed Poisson inter-arrival construction using cubic interpolation \citep{eat_cubic}.
Our general comparator is ReinMax, a quadratic ST estimator for categorical variables \citep{reinmax}; we apply it to count distributions (Poisson, Binomial, and Negative-Binomial) through categorical approximation where feasible and through the Gamma--Poisson representation for Negative-Binomial variables.
For unbounded categorical approximations, we choose the truncation so that the omitted tail has probability at most $0.001$; the appendix gives more detail.
Both comparators have a tuned temperature $\tau$.
We also include EAT-sigmoid, Gumbel--Softmax, and score-function estimators where they are part of the original benchmark comparison. EAT-sigmoid and Gumbel--Softmax require a temperature.

We follow the metrics in prior works for the corresponding benchmarks.
Higher ELBO and lower perplexity are better.
Parenthesized numbers beside temperature-based methods give the selected $\tau$; our estimators and the score-function estimator do not use a temperature.
% Across all tables, boldfacing and underlining mark the best and second-best mean performance in each benchmark.
% \donghan{added bolding and underlying policies here, to avoid repitition in table captions, please review}
% \donghan{people ar elazy add them back}

% \subsection{Linear Poisson VAE: Testing Order-2 Exactness}
% \label{sec:linear-vae}

% \noindent
% \begin{minipage}[t]{0.39\linewidth}
% \vspace{0pt}
% In a Poisson VAE, an encoder specifies a Poisson distribution over latent counts $Z$ given an observation, and a decoder maps those counts back to an observation distribution.
% We use the linear-decoder van Hateren benchmark of \citet{eat_cubic}, which has an analytic gradient for comparison.
% With a Gaussian observation likelihood and a linear decoder, the benchmark's downstream objective is quadratic in the latent counts, so the order-2 estimator is exact here.
% We tune EAT-cubic over its reported temperature grid.
% In Figure~\ref{fig:lin-vae}, the observed mean gradient errors at both checkpoints are near zero, while order 2 has about one-fifth the gradient-error standard deviation of tuned EAT-cubic.
% Its validation-ELBO trajectory also lies closer to the analytic-gradient reference during training.


% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.58\linewidth}
% \vspace{0pt}
% \centering
% \includegraphics[width=\linewidth]{figures/lin_vae_results.png}
% \captionsetup{font=small,skip=3pt}
% \captionof{figure}{Linear Poisson VAE with 512 latent dimensions. \textbf{Left}: mean single-sample gradient error relative to the analytic gradient early in training (epoch 100) and partway through training (epoch 1,000), shown as dots with standard-deviation bars. Both means are near zero; order 2 has about one-fifth the standard deviation of tuned EAT-cubic. \textbf{Right}: validation ELBO over training, mean $\pm$ standard deviation across five matched seeds. Fini-2 follows the analytic-gradient trajectory more closely. 
% % \lw{[For all figures, let’s use .pdf format for higher resolution. Also, increase the font size. Important texts like caption and legends should be roughly the same size of the main text.}
% }
% % \lw{Clarify which scalar gradient error is plotted and how many draws determine each mean and standard deviation.}
% \label{fig:lin-vae}
% \end{minipage}
% \par\medskip

% \input{sections/5.1_lin_pvae_wrap_around}
\input{sections/5.1_lin_pvae_no_wrap}

\FloatBarrier
\subsection{Performances over Realistic Benchmarks}
\label{sec:beyond-matched}

Proposition~\ref{prop:smooth-bias} gives a bias bound outside the prescribed unbiasedness class, but the question remains - can our low-order estimators perform well under realistic benchmarks, where the downstream functions can be nonlinear, and have multiple stochastic layers?

\paragraph{Neural sequence model.}
The partially observed generalized linear model (POGLM) is an autoregressive latent variable model for inferring connectivities from partially observed spike trains. 
As a dynamic graphical model, it has both observed and latent Poissons whose rate parameters depend on recent count histories \citep{second_gsm_poglm}. 
We reproduce the synthetic benchmark in \citet{eat_cubic}, following the same temperature grids and tuning protocol and evaluate 30 matched independent seeds.
% Orders 2, order 3 and the tuned EAT-cubic form a leading group whose displayed means differ by at most $0.02$ (Table~\ref{tab:poglm}); the temperature-free estimators therefore match the tuned specialist on this task.
Table~\ref{tab:poglm} compares validation ELBOs for Fini 2 and 3, EAT-cubic, Gumbel--Softmax, EAT-sigmoid, and the score-function estimator on the synthetic POGLM benchmark. The temperature-free Fini 2 and 3 have mean ELBOs close to tuned EAT-cubic, while the other baselines are worse.

\begin{table}[t]
\centering
\begin{minipage}{\linewidth}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Synthetic POGLM validation ELBO (higher is better), mean $\pm$ standard deviation over 30 matched seeds. Parentheses give the selected temperature $\tau$ for temperature-based estimators. Boldface marks the three highest means, which differ by at most $0.02$.}
\label{tab:poglm}
\centering
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Dataset
& Order 3
& Order 2
& EAT-cubic (0.1)
& GSM (0.5)
& EAT-sigmoid (0.5)
& Score \\
\midrule
Synthetic
& $\mathbf{-330.61\pm0.79}$
& $\mathbf{-330.60\pm0.75}$
& $\mathbf{-330.62\pm0.79}$
& $-331.94\pm0.95$
& $-332.18 \pm 0.97$
& $-333.23 \pm 1.51$ \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}

\paragraph{Nonlinear Poisson VAEs.}
% Following the discrete-VAE setup of \citet{reinmax}, we replace Bernoulli latents with Poisson latents on MNIST, Fashion-MNIST, and Omniglot while retaining the Bernoulli- and Gaussian-likelihood preprocessing protocols;
% \lw{What does "retaining the Bernoulli- and Gaussian-likelihood protocols" mean?}
% \donghan{this is a common benchmark for testing bernoulli and categorical log likelihoods. they preprocess mnist (and fmnist omniglot) in 2 ways: either binarzied dynamically, or whitened into continuous, which corresponds to bernoulli and gaussian.}
Following the discrete-VAE setup of \citet{reinmax}, we evaluate MNIST, Fashion-MNIST, and Omniglot under two data and observation-likelihood settings: dynamically binarized images with a Bernoulli likelihood, and whitened continuous images with a Gaussian likelihood. In both settings, we replace the Bernoulli latent variables with Poisson latent variables (see
\appref{app:nonlinear-count-vae-details} for details). 
\Cref{tab:binary-latent-vae} summarizes results for our method with order 2 and 3, EAT-cubic and ReinMax. Order 3 comes first in 4 out of 6 test cases where order 2 closely follows. Our estimators occupy the leading tier across all six scenarios (Table~\ref{tab:binary-latent-vae}). Order 3 leads in all Bernoulli-likelihood results, while the preferred order varies under Gaussian likelihoods.
This indicates that higher unbiasedness does not result in uniformly better optimization outcomes.

\begin{table}[t]
\centering
\begin{minipage}{\linewidth}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Nonlinear Poisson-VAE training ELBO (higher is better), mean $\pm$ standard deviation over five matched seeds. Columns pair each dataset with a Bernoulli or Gaussian observation likelihood. Parentheses give the selected temperature $\tau$ for temperature-based estimators. 
% Boldface and underlining mark the highest and second-highest mean in each column.
}
\label{tab:binary-latent-vae}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{Bernoulli Likelihoods}
& \multicolumn{3}{c}{Gaussian Likelihoods} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& MNIST
& Fashion-MNIST
& Omniglot
& MNIST
& Fashion-MNIST
& Omniglot \\
\midrule
Order 3
& $\bm{-118.60 \pm 0.26}$
& $\bm{-251.98 \pm 0.40}$
& $\bm{-129.38 \pm 0.07}$
& $\underline{595.48\pm3.72}$
& $\bm{133.74 \pm2.80}$
& $\underline{403.14 \pm 2.46}$ \\

Order 2
& $\underline{-118.88 \pm 0.19}$
& $\underline{-252.26 \pm 0.18}$
& $\underline{-129.93\pm0.12}$
& $594.47\pm3.92$
& $132.09\pm3.29$
& $\bm{403.80 \pm 2.00}$ \\

EAT-cubic
& $-120.06 \pm 0.17$ (0.5)
& $-253.04 \pm 0.22$ (0.5)
& $-130.76 \pm 0.07$ (0.2)
& $\bm{595.66\pm 3.60}$ (0.5)
& $\underline{132.42\pm1.70}$ (0.5)
& $400.84\pm2.05$ (0.5)\\

ReinMax
& $-125.87 \pm 0.38$ (1.1)
& $-260.56 \pm 0.57$ (1.1)
& $-140.07 \pm 0.40$ (1.0)
& $589.21\pm2.78$ (1.0)
& $104.06\pm2.51$ (1.1)
& $396.63 \pm 1.53$ (1.0) \\
\bottomrule
\end{tabular}}
\end{minipage}
\end{table}

\paragraph{Hierarchical topic models.}
We next test our estimators on Deep Exponential Families (DEF), a deep generative model used for topic modeling and recommender systems \citep{def}.
As a hierarchical model, DEF generate observed data through multiple stochastic layers, where each layer drawn from an exponential-family distribution whose natural parameters are determined by the previous layer. 
We train amortized two-layer sparse Poisson DEFs on 20 Newsgroups (20 NG) and RCV1 using the inference architecture of \citet{nvil}; \appref{app:DEF-deets} gives the full setup. 

\begin{table}[t]
\centering
\begin{minipage}{\linewidth}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Poisson DEF results, mean $\pm$ standard deviation over five matched seeds. Higher is better for training and test ELBO; lower is better for held-out perplexity (PPL). Parentheses give the selected temperature $\tau$ for EAT-cubic and ReinMax. Bolded and underlined are the first and the second.
% Boldface and underlining mark the best and second-best mean for each metric and dataset; tied means share a rank.
}
% \lw{What is EA-cubic(0.2) and ReinMax(1.3)?}
\label{tab:topic-modeling-perplexity}
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccc@{\hspace{6pt}}ccc@{}}
\toprule
&
& \multicolumn{3}{c}{20 Newsgroups}
& \multicolumn{3}{c}{RCV1} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
Model
& Training method
& Train ELBO $\uparrow$
& Test ELBO $\uparrow$
& PPL $\downarrow$
& Train ELBO $\uparrow$
& Test ELBO $\uparrow$
& PPL $\downarrow$ \\
\midrule
\multirow{4}{*}{Poisson DEF}
& Order 3
& $\bm{-179.30 \pm 2.81}$
& $\underline{-199.31 \pm 2.04}$
& $660.7 \pm 7.6$
& $\underline{-269.27 \pm 3.16}$
& $\underline{-267.64 \pm 3.73}$
& $\bm{379.3 \pm 5.4}$ \\

& Order 2
& $\bm{-179.30 \pm 2.62}$
& $\bm{-198.98 \pm 1.92}$
& $\underline{659.7 \pm 6.7}$
& $\bm{-269.20 \pm 3.05}$
& $\bm{-267.60 \pm 3.73}$
& $\underline{381.9 \pm 4.6}$ \\

& EAT-cubic (0.2)
& $\underline{-180.94 \pm 2.59}$
& $-199.77 \pm 2.17$
& $664.6 \pm 8.5$
& $-271.92 \pm 3.18$
& $-270.16 \pm 3.82$
& $388.4 \pm 4.1$ \\

& ReinMax (1.3)
& $-191.25 \pm 2.88$
& $-210.01 \pm 2.37$
& $\bm{638.1 \pm 10.5}$
& $-301.86 \pm 2.83$
& $-300.05 \pm 3.27$
& $384.4 \pm 4.8$ \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\end{table}


\Cref{tab:topic-modeling-perplexity} summarize the results.
Fini 2 and 3 have the two highest mean train and test ELBOs on both datasets. Held-out perplexity ranks the methods differently: ReinMax leads on the smaller 20 NG dataset, whereas order 3 leads on RCV1.
To diagnose why ReinMax leads on 20 NG but not on RCV1, we split the ELBO loss into the log likelihood dimension and the KL divergence dimension, and use the expensive but low variance MVD gradients as a ground truth to compare against.
% and compute each method's gradient with respect to each dimension at respective optimums.
% Furthermore, we use the unbiased, low variance but computationally expensive MVD gradients \cite{mvd} as a near-exact ground truth for comparison.
We found that ReinMax at $\tau= 1.3$ highly biases towards worse KL, and better log likelihood (which highly correlates with perplexity), while our methods closely track the MVD gradients for both datasets; 
% Thus, the takeaway is that our estimator stays faithful to the model's exact gradient, while ReinMax biases towards lower log likelihood, which correlates with better perplexity; 
so ReinMax's win in held out perplexity on the smaller 20 NG dataset is a byproduct of its bias.
For the detailed diagnostic, please see \appref{app:def-rate-distortion}. 

\paragraph{Summary.} Across these nonlinear and hierarchical tasks, our order 2 and 3 estimators matches tuned EAT-cubic on POGLM and improves it on most ELBOs.
Both orders outperform ReinMax on every displayed ELBO, although the preferred order remains task dependent. 
The heldout perplexity metric shows the more biased ReinMax method resulted in better performance in the smaller dataset; but further investigation shows that this is a byproduct of the method's bias, not better gradients.

% \FloatBarrier
\subsection{Generality Across Common Discrete Variables}
\label{sec:nonlinear-vae-more}

We next ask whether the performance applies across Poisson, Binomial, and Negative-Binomial variables and varying latent dimensions on MNIST. 
To test this, we use these discrete variables as the latent variable in VAEs and vary the latent dimension across $[2,16,128]$.
For Poisson and Binomial, ReinMax can work with categorical embedding up to truncation. 
For Negative Binomial, direct truncation is impractical as the distribution is over-disperse, which means the number of states we need to represent it is too large; so we have to apply ReinMax through the Gamma--Poisson representation(Table~\ref{tab:mnist-count-vae-train}).
Results are shown in \ref{tab:mnist-count-vae-train}, order 3 estimator leads at higher latent dimensions, while order 2 leads in two of the three 2-dimensional settings, again making exactness order a problem-dependent choice rather than a fixed ranking.

\begin{table}[t]
\centering
\begin{minipage}{0.88\linewidth}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Count-VAE training ELBO, mean $\pm$ standard deviation over five independent matched seeds. Selected ReinMax temperatures appear in parentheses.}
\label{tab:mnist-count-vae-train}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.02}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
Family
& Latent dim.
& Order 2
& Order 3
& ReinMax \\
\midrule
\multirow{3}{*}{\shortstack[l]{binomial\\$n=8, p=0.5$}}
& 2
& $\mathbf{-174.51 \pm 0.45}$
& $\underline{-176.91 \pm 1.07}$
& $-179.67 \pm 0.67$ (1.0) \\
& 16
& $\underline{-123.38 \pm 0.14}$
& $\mathbf{-123.11 \pm 0.10}$
& $-125.55 \pm 0.10$ (1.0) \\
& 128
& $\underline{-118.73 \pm 0.22}$
& $\mathbf{-118.43 \pm 0.17}$
& $-121.45 \pm 0.15$ (1.1) \\
\midrule
\multirow{3}{*}{\shortstack[l]{negbin\\$r=8, p=0.5$}}
& 2
& $\underline{-177.34 \pm 0.15}$
& $\mathbf{-177.31 \pm 0.24}$
& $-182.58 \pm 0.48$ (1.0) \\
& 16
& $\underline{-129.29 \pm 0.16}$
& $\mathbf{-129.25 \pm 0.20}$
& $-136.58 \pm 0.71$ (1.0) \\
& 128
& $\underline{-122.58 \pm 0.06}$
& $\mathbf{-122.54 \pm 0.36}$
& $-124.41 \pm 0.24$ (1.1) \\
\midrule
\multirow{3}{*}{\shortstack[l]{poisson\\$\lambda_0=0.1$}}
& 2
& $\mathbf{-190.37 \pm 0.66}$
& $\underline{-191.77 \pm 1.57}$
& $-199.33 \pm 2.57$ (1.0) \\
& 16
& $\underline{-146.74 \pm 0.62}$
& $\mathbf{-145.68 \pm 0.31}$
& $-170.60 \pm 0.39$ (1.0) \\
& 128
& $\underline{-123.20 \pm 0.30}$
& $\mathbf{-122.80 \pm 0.40}$
& $-129.99 \pm 1.02$ (1.0) \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\end{table}

\paragraph{Compound representation adds statistical overhead.}
For Negative-Binomial latents, a Gamma--Poisson construction reuses a Poisson estimator by introducing an auxiliary rate $\Lambda$ before sampling $Z$.
Corollary~\ref{cor:gamma-poisson} predicts two distinct consequences: at order 2, conditioning on $Z$ exactly recovers the native weight, so all excess weight variance comes from the auxiliary Gamma variable; at order 3, conditioning can leave a nonminimal $Z$-only component.
We reproduce the variance study from \citep{disarm}, and replace the latent Bernoulli with Negative-Binomial.
The 128-dimensional Negative-Binomial variance study results are shown in Figure~\ref{fig:rb-exp}.
The results support our variance ordering theory: each native order has lower gradient variance than its matched Gamma--Poisson compound estimator, while the non-native ReinMax has higher variance.

% \FloatBarrier
\begin{figure}[t]
\centering
\begin{minipage}{0.92\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/gvar_negbin_revised.png}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Negative-Binomial representation diagnostic. Native order-2 and order-3 estimators have lower gradient variance than their matched Gamma--Poisson compound counterparts; ReinMax has higher variance and a larger discrepancy from native order 2 in the displayed run.}
\label{fig:rb-exp}
\end{minipage}
\end{figure}

\noindent
\begin{minipage}[t]{0.60\linewidth}
\vspace{0pt}
\textbf{Categorical representation adds computational overhead.}
For Binomial latents, the released hard 1D MVE implementation of \citet{hooperetal2026} operates over $K=n+1$ categorical states, whereas our fixed-order weights' costs are independent of the support size.
Figure~\ref{fig:binom-mve-support-scaling} shows the resulting support-size scaling.
The compound and categorical results therefore test different costs of non-native representations: statistical overhead from auxiliary variables and computational overhead from categorical embedding.
\end{minipage}
\hfill
\begin{minipage}[t]{0.36\linewidth}
\vspace{0pt}
\centering
\includegraphics[width=\linewidth,]{figures/binom_timing.png}
\captionsetup{font=footnotesize,skip=3pt}
\captionof{figure}{Categorical support scaling. At $n=1024$, the released 1D MVE implementation takes $38\times$ as long as native order 2. } 
\label{fig:binom-mve-support-scaling}
\end{minipage}
\par\medskip

% \FloatBarrier
\subsection{Speed Comparisons}
\label{sec:comp-speed}

Fixed-order Fini weights require one forward--backward pass and evaluates affine or quadratic polynomials.
Across three benchmarks on L4 and A100 GPUs, Fini order 2 and 3 are first and second in every workload--hardware pair (Table~\ref{tab:speed-results}); \appref{app:timing-details} gives the five-repeat post-warm-up protocol.
Order 2 is consistently faster because it evaluates an affine rather than quadratic weight.

\begin{table}[t]
\centering
\begin{minipage}{\linewidth}
\captionsetup{font=footnotesize,skip=3pt}
\caption{Wall-clock seconds per epoch ($\downarrow$), mean $\pm$ standard deviation over five timing repeats.}
\label{tab:speed-results}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{Linear VAE}
& \multicolumn{2}{c}{Nonlinear VAE}
& \multicolumn{2}{c}{DEF} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Estimator
& L4 & A100
& L4 & A100
& L4 & A100 \\
\midrule
Order 3
& $\underline{0.326 \pm 0.010}$
& $\underline{0.361 \pm 0.008}$
& $\underline{1.868 \pm 0.074}$
& $\underline{2.016 \pm 0.083}$
& $\underline{0.928 \pm 0.021}$
& $\underline{0.907 \pm 0.016}$ \\
Order 2
& $\bm{0.309 \pm 0.005}$
& $\bm{0.338 \pm 0.004}$
& $\bm{1.768 \pm 0.017}$
& $\bm{1.848 \pm 0.046}$
& $\bm{0.863 \pm 0.014}$
& $\bm{0.835 \pm 0.016}$ \\
EAT-cubic
& $1.427 \pm 0.005$
& $0.581 \pm 0.010$
& $2.680 \pm 0.040$
& $2.942 \pm 0.073$
& $1.546 \pm 0.039$
& $1.565 \pm 0.015$ \\
ReinMax
& $1.144 \pm 0.006$
& $0.568 \pm 0.009$
& $2.692 \pm 0.035$
& $2.859 \pm 0.104$
& $1.451 \pm 0.024$
& $1.610 \pm 0.134$ \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\end{table}
\FloatBarrier


==> sections/5.1_lin_pvae_wrap_around.tex <==
\subsection{Linear Poisson VAE: Testing Order-2 Exactness}
\label{sec:linear-vae}

\begin{wrapfigure}{r}{0.58\textwidth}
    \vspace{-0.6\baselineskip}
    \centering
    \includegraphics[width=\linewidth]{figures/lin_vae_results.png}
    \captionsetup{font=small,skip=3pt}
    \caption{Linear Poisson VAE with 512 latent dimensions.
    \textbf{Left}: mean single-sample gradient error relative to the
    analytic gradient early in training (epoch 100) and partway through
    training (epoch 1,000), shown as dots with standard-deviation bars.
    Both means are near zero; Fini-2 has about one-fifth the standard
    deviation of tuned EAT-cubic.
    \textbf{Right}: validation ELBO over training, mean $\pm$ standard
    deviation across five matched seeds. Fini-2 follows the
    analytic-gradient trajectory more closely.}
    \label{fig:lin-vae}
    \vspace{-0.5\baselineskip}
\end{wrapfigure}

In a Poisson VAE, an encoder specifies a Poisson distribution over latent
counts $Z$ given an observation, and a decoder maps those counts back to an
observation distribution.
We use the linear-decoder van Hateren benchmark of \citet{eat_cubic}, which
has an analytic gradient for comparison.
With a Gaussian observation likelihood and a linear decoder, the benchmark's
downstream objective is quadratic in the latent counts, so Fini-2 is exact here.
We tune EAT-cubic over its reported temperature grid.
In Figure~\ref{fig:lin-vae}, the observed mean gradient errors at both
checkpoints are near zero, while Fini-2 has about one-fifth the gradient-error
standard deviation of tuned EAT-cubic.
Its validation-ELBO trajectory also lies closer to the analytic-gradient
reference during training.

==> sections/6.0_limitations.tex <==
\section{Limitations}
\label{sec:limitations}
\lw{If running out of space, can merge limitations and conclusion to a Discussion section in two separate paragraphs.}

Our discrete pathwise extension framework requires the relevant moments and their parameter derivatives, and degree-$D$ exactness requires at least $D$ support points.
Applying the framework to a new distribution therefore still requires deriving or computing these quantities.
Outside the matched polynomial class, the bias bound also requires the smoothness and moment conditions of Proposition~\ref{prop:smooth-bias}; polynomial unbiasedness alone does not guarantee small bias.
Finally, higher $D$ adds an orthogonal correction and cannot decrease
the weight's raw second moment; the fourth-order Poisson example in
\appref{app:poisson-order4} shows that its variance can deteriorate sharply
at low rates.
Thus, estimator order controls a bias--variance tradeoff rather than
providing a uniform improvement.


==> sections/7.0_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Polynomially exact least-norm estimation makes approximation order an explicit design parameter for same-path discrete gradients.
% Prescribing degree-$D$ exactness yields a finite moment problem, while least-norm selection gives the unique minimum-weight-variance solution within that exactness class.
% For common discrete laws, the resulting native polynomial weights preserve the exact forward sample, require one downstream forward--backward pass, and use neither temperature tuning nor auxiliary randomness.
% The theory extends exactness on matched polynomials to smooth downstream functions through a non-asymptotic bias bound and identifies orthogonal null components as the source of excess weight variance.
% Empirically, orders 2 and 3 remain in the leading performance tier across increasingly realistic benchmarks, while ranking first and second in every runtime benchmark.
% The resulting family makes the bias--variance--computation tradeoff explicit: approximation order can be chosen directly rather than inherited from a relaxation or estimator construction.
We extend pathwise gradients to discrete distributions by prescribing degree-$D$ polynomial exactness \lw{mention the polynomial context} and then choosing the least-norm solution.
% This recipe recovers classical pathwise results such as location--scale family gradients and the minimum-energy Gaussian vector pathwise field.
For common discrete variables, the resulting polynomial weights preserve the exact forward sample, require one %downstream 
forward--backward pass, and use neither temperature tuning nor auxiliary randomness.
Moreover, this recipe recovers classical pathwise gradients for continuous random variables.
Our theory extends the guarantees beyond exactness class through a non-asymptotic bias bound for smooth functions and decomposes excess weight variance into auxiliary-variable noise and orthogonal null components.
Empirically, orders 2 and 3 remain in the leading performance tier across increasingly realistic benchmarks, while ranking first and second in every runtime benchmark. 
% Thus, we recommend using our estimators as a default for common discrete distributions, for they are low-bias, low-variance, low-compute, and easy to implement. 
% \lw{Let's temper the recommendation; instead, state the desirable properties / advantages.}
Thus, we provide a general derivation principle for extending pathwise gradient estimators beyond continuous random variables, yielding low-bias, low-variance, low-compute and simple to implement estimators.


==> sections/8.0_disclosures.tex <==
\section*{AI statement:}
We used LLMs to periodically and systematically search for related work.
We used LLM to improve paper organization and grammar, but not to generate full sections from scratch.
We also used LLM to reorganize human-written proofs and math prose into more concise statements.
All LLM assisted text and codes have been verified by us, and we take full responsibility for the end results.

\section*{Ethics statement:}
This work develops a general-purpose gradient estimation method and does not involve human subjects or sensitive data. 
Its reduced computational overhead may lower barriers to experimenting with discrete latent-variable models, though we do not directly measure monetary or environmental costs.

\section*{Reproducibility statement:}
We show worked-out estimator formulas for all variables in \appref{app:estimators}, a torch implementation in \Cref{lst:intro-poisson} and multi-parameter implementation in \appref{sec:two-parameter-st}.
We provide all experiment details in \appref{app:experiments}.
We plan to release the code after the review process.
